All-in-One: A Highly Representative DNN Pruning Framework for Edge Devices with Dynamic Power Management

During the deployment of deep neural networks (DNNs) on edge devices, many research efforts are devoted to the limited hardware resource. However, little attention is paid to the influence of dynamic power management. As edge devices typically only have a budget of energy with batteries (rather than almost unlimited energy support on servers or workstations), their dynamic power management often changes the execution frequency as in the widely-used dynamic voltage and frequency scaling (DVFS) technique. This leads to highly unstable inference speed performance, especially for computation-intensive DNN models, which can harm user experience and waste hardware resources. We firstly identify this problem and then propose All-in-One, a highly representative pruning framework to work with dynamic power management using DVFS. The framework can use only one set of model weights and soft masks (together with other auxiliary parameters of negligible storage) to represent multiple models of various pruning ratios. By re-configuring the model to the corresponding pruning ratio for a specific execution frequency (and voltage), we are able to achieve stable inference speed, i.e., keeping the difference in speed performance under various execution frequencies as small as possible. Our experiments demonstrate that our method not only achieves high accuracy for multiple models of different pruning ratios, but also reduces their variance of inference latency for various frequencies, with minimal memory consumption of only one model and one soft mask.

==> tex/method_1.tex <==
\section{Parametric Pruning one}
\begin{prop}
The error of each sub-network $g(\mathbf{x}; (\mathbf{P}\odot\mathbf{W})\odot \mathbf{M})$ within the multi-device sparse model $g(\mathbf{x}; (\mathbf{P}\odot\mathbf{W}))$ is upper bounded by the sum of the connectivity error $L \| \mathbf{W} \odot (\mathbf{M}-\mathbf{P})\|$ and the pattern error $\|g(\mathbf{x}; (\mathbf{P}\odot\mathbf{W})) - f(\mathbf{x}; \mathbf{W}^*)\|$. (not finished)
\end{prop}
\begin{proof}
Let $f(\mathbf{x}; \mathbf{W}^*)$ be any optimized dense model with weights $\mathbf{W}^*$, which is the target for the sub-network $g(\mathbf{x}; (\mathbf{P}\odot\mathbf{W})\odot \mathbf{M})$ to approximate, where $\mathbf{P}$ represents the pattern mask, $\mathbf{M}$ is the connectivity mask, and $\odot$ is the  Hadamard product. Assuming $g(\mathbf{x};\cdot)$ is $L$-Lipschitz  continuous, for a fixed Lipschitz constant $L > 0$, it yields 
\begin{align}
     & \| g(\mathbf{x}; (\mathbf{P}\odot\mathbf{W})\odot \mathbf{M}) - f(\mathbf{x}; \mathbf{W}^*) \|  \\
     \leq &   \| g(\mathbf{x}; (\mathbf{P}\odot\mathbf{W})\odot \mathbf{M}) - g(\mathbf{x}; (\mathbf{P}\odot\mathbf{W})) \| + \notag \\ 
     & \| g(\mathbf{x}; (\mathbf{P}\odot\mathbf{W})) - f(\mathbf{x}; \mathbf{W}^*) \| \\
     \leq &   L \| \mathbf{W} \odot (\mathbf{P}\odot\mathbf{M}-\mathbf{P})\| + \| g(\mathbf{x}; (\mathbf{P}\odot\mathbf{W})) - f(\mathbf{x}; \mathbf{W}^*) \| \label{eq:lipschitz}
\end{align}
As connectivity pruning is applied after pattern pruning, i.e., $\mathbf{P}\odot\mathbf{M}$ is equivalent to $\mathbf{M}$, we can get 
\begin{align}
     & \| g(\mathbf{x}; (\mathbf{P}\odot\mathbf{W})\odot \mathbf{M}) - f(\mathbf{x}; \mathbf{W}^*) \| \notag \\
    \leq & \underbrace{L \| \mathbf{W} \odot (\mathbf{M}-\mathbf{P})\|}_{\textrm{connectivity error}} + \underbrace{\| g(\mathbf{x}; (\mathbf{P}\odot\mathbf{W})) - f(\mathbf{x}; \mathbf{W}^*) \|}_{\textrm{pattern error}} \label{eq:c_p_error}
\end{align}
\end{proof}

Based on Eq. (\ref{eq:c_p_error}), and $\mathbf{P}$ is a fixed mask, we can formulate a minimization problem to optimize the connectivity mask $\mathbf{M}$ generated by score $\mathbf{S}$ using $\ell_2$ norm as

\begin{equation}
    \min \| \mathbf{W} \odot (\mathbf{M}-\mathbf{P})\|_{2}.
\end{equation}
Let $\mathbf{U}_l=(\mathbf{M}_l \odot \mathbf{W}_l)\mathbf{x}_l$ represents the output of the $l$-th layer, we have $ \frac{\partial\mathcal{L}}{\partial{S}_l} = \frac{\partial\mathcal{L}}{\partial \mathbf{U}_l} \frac{\partial \mathbf{U}_l}{\partial{M}_l}\frac{\partial \mathbf{M}_l}{\partial{S}_l}$.
